Auto-SPT: Automating Semantic Preserving Transformations for Code

Machine learning (ML) models for code clone detection determine whether two pieces of code are semantically equivalent, which in turn is a key building block for software-engineering tasks like refactoring and security tasks like vulnerability and malware detection. While these models are predominantly trained on clean, structured code datasets, real-world code often undergoes a variety of semantic-preserving transformations, including refactoring, minification, automated formatting, and compiler optimizations. To address this critical gap between training and test data, we propose Auto-SPT, a novel framework to automatically construct synthetic-data generators for code. Auto-SPT is designed to produce Semantic Preserving Transformations (SPTs) that alter a program's syntactic structure while preserving its functionality and is instantiated on top of Large Language Models (LLMs). In particular, we use LLMs to craft a diverse set of SPTs, generate strong implementations for these SPTs, and compose them to result into strong transformations. Our formal analysis shows that the diversity of SPTs impacts the strength of their composition. We then empirically demonstrate that Auto-SPT generates more diverse SPTs than existing approaches and these SPTs significantly drop the performance of state-of-the-art code clone detectors. Further experiments show Auto-SPT can be used to enhance code datasets for training, to produce code-clone detection models that are robust to real-world, adversarial code transformations.

==> 05_evaluation.tex <==
\section{Experiments}
\label{sec:eval}
Our evaluation answers the following research questions:

\noindent\textbf{RQ1:} How diverse are \name's SPTs as compared to existing transformations?

\noindent\textbf{RQ2:} How effective is \name at evading clone detectors as compared to existing transformations?







\noindent\textbf{RQ3:} How does \name perform against robust clone detectors?

\subsection{Setup}
\paragraph{Dataset.} We use the CodeContests dataset from~\cite{li2022competition} to construct clone and non-clones code pairs. Each problem in this dataset comes with multiple solutions (submitted by actual users via platforms like Codeforces, CodeChef, etc.) as well as unit tests. We use solutions belonging to the same problem to construct clone pairs and those belonging to distinct problems to construct non-clone pairs. In total, we randomly select $2000$ distinct problems. Then, we split this to get $1500$ training, $250$ validation, and $250$ test sets of problems. The split is done to test the generalization performance of the clone detection task across different functionalities. Now, for each set, we construct $250$ clone pairs per problem, leading to a total of $375000$ clone pairs in the training set. We construct an equal number of non-clone pairs to get a balanced dataset. We ensure that we only consider solutions that pass all the unit tests associated with the corresponding problem. In this
evaluation, we focus on Python programs, but our methodology applies to any programming language.

\paragraph{Clone Detection Models.} We evaluate \name using three different model architectures -- CodeBERT, GraphCodeBERT, and Starencoder. We perform full finetuning for the CodeBERT model using the training set and select the best checkpoint based on the accuracy of the validation set. For the other models, we use the pretrained weights and fine-tune the final layer. For both settings, we train for at most $10$ epochs.

\paragraph{\name Hyperparameters.} We use Gemini 2.5 Pro for both designing and implementing SPTs (i.e., as the LLM for Steps 1 and 2 of \name). We use a temperature of $0.1$ for the design step and $0.8$ for the implementation step. We use the remaining solutions from CodeContest (disjoint from the $2000$ problems considered during dataset generation) to populate the example programs in the generator prompt. We use $N=20$ for Best-of-N sampling during the implementation step. Again, we sample the validation programs to estimate the reward function from the remaining CodeContest solutions. For the beam search, we use a beam size of $5$ and apply each SPT to all the candidates in the beam. For RQ1 and RQ3, we run the beam size for $50$ iterations. For RQ1, we only run the search for $10$ steps due to computational reasons. We use the following notation to denote different transformation sets. \texttt{VarRename}, \texttt{Conditional}, \texttt{ForWhile} and \texttt{IfElseFlip} are together described as \texttt{Orig-4}. The transformations mentioned in Table 1 are represented by \texttt{New-20}. 


\paragraph{Compute.} We run all experiments on a machine with 4 NVIDIA H100 GPUs, 40 Intel(R) Xeon(R) Silver 4410T CPUs, and 126GB of RAM. Full finetuning of CodeBERT took around 24 hours due to the small batch size used in the original training recipe. For a transformation set of size 4, a 50-step beam search took around 1 hour.

\subsection{RQ1: Transformation Set Diversity}
We use the search procedure described in \autoref{sec:beam} to estimate the diversity (\autoref{def:divesity}) of a set of transformations. In \autoref{fig:diversity}, we show the diversity values for an increasing number of implementations from two different sets of transformations -- \texttt{Orig-4}, and \texttt{New-20}. To expand the \texttt{Orig-4} set to 20 implementations, we use \name to generate multiple implementations for each SPT type. Due to the high computation cost of estimating diversity, we limit the maximum number of search iterations to $5$ (since estimating diversity for a set of $k$ transformations requires running $k$ search procedures). We see that the diversity of \texttt{Orig-4} goes down rapidly as the number of transformations increases. Going from $12$ to $16$ transformations has a minimal effect on the transformation strength. On the other hand, \texttt{New-20} maintains diversity even for $20$ transformations. This result highlights \name's ability to design diverse SPTs.

\input{table_individual}


\subsection{RQ2: Attack Effectiveness}
\autoref{tab:multi_model} shows distance measured by the clone detector model for the worst-case transformation against three different types of clone detection models. For the search, we consider four different settings which correspond to four different sets of SPTs and their implementations --\cite{wang2022recode} (\texttt{Orig-4}), \name (\texttt{Orig-4}), \name (\texttt{Orig-20}) and \name (\texttt{New-20}), where the third type is constructed by taking distinct implementations (4 each) of the \texttt{Orig-4} transformations. Across the three models, we make two main observations: (1) For the same type of transformations, \name outperforms implementations provided by past work, and (2) SPTs designed by \name can be composed to perform stronger transformations as compared to existing SPTs.  

\input{table_multiple_models} 

\subsection{RQ3: Evaluating Robust Detectors}
Next, we evaluate the effectiveness of \name against clone detectors that are trained to be robust to SPTs. We finetune additional settings of CodeBERT where we augment the training data by applying transformations from \texttt{Orig-4}. We consider two settings -- SPT implemented by \cite{wang2022recode} and \name. We decide to transform each training point with a probability of $0.5$, and then select a random SPT from the transformation set. \autoref{fig:adv} shows the transformation effectiveness for all three settings. First, we find that training on transformations from \cite{wang2022recode} improves robustness the most against the same transformation set. It provides minor improvements against \texttt{Orig-4} or \texttt{New-20} transformations from \name. However, training on \texttt{Orig-4} transformations from \name improves robustness against both \cite{wang2022recode} and \name's implementations. It slightly improves against \texttt{New-20} transformations, suggesting that training on stronger transformations helps improve robustness against weaker transformations of the same type.

\input{adv_runs}

==> table_comparison.tex <==
\begin{table}
\scriptsize
\centering
\caption{Performing SPTs using LLMs. }
\label{tab:spt}
\begin{tabular}{lcccccc}
\toprule
\textbf{SPT} & \textbf{Total Programs} & \textbf{Pass Tests - Symbolic} & \textbf{Pass Tests - LLM} & \textbf{Exact Match} & \textbf{Diff < 10\%} & \textbf{Diff < 30\%}\\
\midrule
\texttt{ForToWhile} & 1000 & 779 & 917 & 475 & 571 & 833 \\
\texttt{IfElseFlip} & 1000 & 989 & 866 & 493 & 713 & 990 \\

\bottomrule

\end{tabular}
\end{table}



==> table_new_individual.tex <==
\begin{table}
\scriptsize
\centering
\caption{New SPTs.}
\label{tab:spt-indiv}
\begin{tabular}{llcc}
\toprule
\textbf{Transformation} & \textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}}\textbf{Equivalence} \\ \textbf{(1000 programs)}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\textbf{Strength} \\ \textbf{($1 - M(x, x')$)}\end{tabular}}\\
\midrule
\texttt{MapToComprehension} & Neuro-Symbolic  & 99.9\% & 0.004 (0.077) \\
\texttt{SliceToLoop} & Neuro-Symbolic  & 52.5\% & 0.002 (0.038) \\
\texttt{FunctionOutlining} & Neural  & 99.1\% & 0.225 (0.395) \\
\bottomrule

\end{tabular}
\end{table}
